Doomed to Re-Annotate, Forever: The ImageNet Story

Top-1 accuracy on ImageNet-1k remains the most commonly reported metric in visual recognition. Quality issues with the dataset have been repeatedly reported, yet the original 2012 noisy labels are still predominantly used. The paper presents a comprehensive effort, which goes well beyond prior correction attempts, towards obtaining accurate and complete ImageNet-1k validation set annotations. The result, ReImageNet, includes multilabel correction, object localization, revised class definitions, and semantic attributes (text-recognition, rendition, reflection, crowd, dominant). The reannotation reveals that approximately 12% of the original ImageNet-1k labels are incorrect, 33.3% of images are multilabel and 3.8% contain no object from an ImageNet-1k class. With the new labels, top-1 accuracy increases by up to 1.2% for supervised models and by 5-6% for MLLMs. We argue that annotation at ImageNet scale cannot realistically be completed in one pass, as errors and definitional issues are discovered only through annotating, and we build our pipeline around repeated refinement and error checking. We observed that human and LLM collaboration with appropriate tooling represents the current quality ceiling for annotation at this scale. ImageNet-1k issues propagate into its derivative test sets, indicating that the problem is structural rather than specific to any single benchmark. All annotations, class definitions, guidelines, and analysis code have been publicly released. Project page: https://vrg.fel.cvut.cz/reimagenet Annotations: https://huggingface.co/datasets/vrg-prague/ReImageNet Code: https://github.com/klarajanouskova/ImageNet

==> tables/additional_sets.tex <==
\begin{table}[t]
    \caption{Results on additional ImageNet test sets.}
    \label{tab:additional_sets_2}
    \small
    % \setlength{\tabcolsep}{3.8pt}
    \begin{tabular}{lrr rrr rrr rr}
        \toprule
        & & & \multicolumn{2}{c}{\cgpt}
            & \multicolumn{2}{c}{\sigliptwog}
            & \multicolumn{2}{c}{\effnetl} \\
        \cmidrule(lr){4-5}
        \cmidrule(lr){6-7}
        \cmidrule(lr){8-9}
        Dataset & \# Cls. & \# Imgs. & In1k & Subset
                                      & In1k & Subset
                                      & In1k & Subset \\
        \midrule
        ImageNetV2      & 1000 & 10{,}000 & 64.13 & 64.13 & 80.24 & 80.24 & 81.42 & 81.42 \\
        ImageNet-A      & 200  & 7{,}500  & 45.13 & 57.25 & 74.69 & 89.57 & 61.73 & 84.65 \\
        ImageNet-R      & 200  & 30{,}000 & 76.89 & 84.05 & 85.95 & 95.44 & 56.64 & 74.61 \\
        ImageNet-Sketch & 1000 & 50{,}889 & 55.15 & 55.15 & 77.00 & 77.00 & 48.03 & 48.03 \\
        ObjectNet       & 125  & 18{,}574 & 68.01 & 72.35 & 74.10 & 80.87 & 61.07 & 69.67 \\
        CounterAnimal   & 45   & 13{,}334 & 75.45 & 86.61 & 91.05 & 94.98 & 90.30 & 93.22 \\
        \bottomrule
    \end{tabular}
\end{table}
